Multiple evolutionary pressures shape identical consonant avoidance in the world's languages

Languages disfavor word forms containing sequences of similar or identical consonants, due to the biomechanical and cognitive difficulties posed by patterns of this sort. However, the specific evolutionary processes responsible for this phenomenon are not fully understood. Words containing sequences of identical consonants may be more likely to arise than those without; processes of word form mutation may be more likely to remove than create sequences of identical consonants in word forms; finally, words containing identical consonants may die out more frequently than those without. Phylogenetic analyses of the evolution of homologous word forms indicate that words with identical consonants arise less frequently than those without, and processes which mutate word forms are more likely to remove sequences of identical consonants than introduce them. However, words with identical consonants do not die out more frequently than those without. Further analyses reveal that forms with identical consonants are replaced in basic meaning functions more frequently than words without. Taken together, results suggest that the under representation of sequences of identical consonants is overwhelmingly a byproduct of constraints on word form coinage, though processes related to word usage also serve to ensure that such patterns are infrequent in more salient vocabulary items. These findings clarify previously unknown aspects of processes of lexical evolution and competition that take place during language change, optimizing communicative systems.

==> cognate-concept-CIs.tex <==
%<*birthRate>
Dravidian: $17.85$, [$6.03$, $35.98$]; Indo-European: $15.85$, [$7.36$, $29.69$]; Sino-Tibetan: $26.56$, [$13.33$, $46.81$]; Turkic: $11.59$, [$3.41$, $27.09$]; Uto-Aztecan: $21.95$, [$9.47$, $47.15$]
%</birthRate>
%<*gainRate>
Dravidian: $1.77$, [$0.18$, $4.81$]; Indo-European: $7.14$, [$1.55$, $15$]; Sino-Tibetan: $5.66$, [$0.95$, $11.81$]; Turkic: $1.38$, [$0.17$, $3.76$]; Uto-Aztecan: $1.7$, [$0.25$, $3.67$]
%</gainRate>
%<*deathRate>
Dravidian: $6.11$, [$3.59$, $9.59$]; Indo-European: $6.67$, [$4.65$, $9.36$]; Sino-Tibetan: $4.68$, [$3.27$, $6.44$]; Turkic: $49$, [$16.56$, $118.88$]; Uto-Aztecan: $4.77$, [$2.65$, $8.34$]
%</deathRate>
%<*birthPairs>
Dravidian: 0/4278; Indo-European: 0/4560; Sino-Tibetan: 1/3403; Turkic: 83/4005; Uto-Aztecan: 0/4186
%</birthPairs>
%<*gainPairs>
Dravidian: 0/4278; Indo-European: 30/4560; Sino-Tibetan: 48/3403; Turkic: 2/4005; Uto-Aztecan: 6/4186
%</gainPairs>
%<*deathPairs>
Dravidian: 1469/4278; Indo-European: 2122/4560; Sino-Tibetan: 2038/3403; Turkic: 666/4005; Uto-Aztecan: 2132/4186
%</deathPairs>
%<*birthRateIndividual>
Dravidian: 0/93, Indo-European: 0/96, Sino-Tibetan: 0/83, Turkic: 47/90, Uto-Aztecan: 0/92
%</birthRateIndividual>
%<*deathRateIndividual>
Dravidian: 5/93, Indo-European: 2/96, Sino-Tibetan: 1/83, Turkic: 7/90, Uto-Aztecan: 1/92
%</deathRateIndividual>
%<*gainRateIndividual>
Dravidian: 93/93, Indo-European: 85/96, Sino-Tibetan: 77/83, Turkic: 90/90, Uto-Aztecan: 92/92
%</gainRateIndividual>

